Distributed Dual Subgradient Methods with Averaging and Applications to Grid Optimization

We study finite-time performance of a recently proposed distributed dual subgradient (DDSG) method for convex constrained multi-agent optimization problems. The algorithm enjoys performance guarantees on the last primal iterate, as opposed to those derived for ergodic means for vanilla DDSG algorithms. Our work improves the recently published convergence rate of $\Ocal(\log T/\sqrt{T})$ with decaying step-sizes to $\Ocal(1/\sqrt{T})$ with constant step-size on a metric that combines suboptimality and constraint violation. We then numerically evaluate the algorithm on three grid optimization problems. Namely, these are tie-line scheduling in multi-area power systems, coordination of distributed energy resources in radial distribution networks, and joint dispatch of transmission and distribution assets. The DDSG algorithm applies to each problem with various relaxations and linearizations of the power flow equations. The numerical experiments illustrate various properties of the DDSG algorithm--comparison with vanilla DDSG, impact of the number of agents, and why Nesterov-style acceleration fails in DDSG settings.

==> introduction_power.tex <==
%!TEX root = MainDistOptPower.tex



\section{Introduction}
\label{sec:intro}
We consider optimization problems that arise in power system operation, where collecting all data at a central location to solve the  problem is not an option. Barriers to such data aggregation can arise due to lack of jurisdiction of one entity over all data sources, or in the interest of speed. In such applications, one must rely on \emph{distributed} solution architectures. Such a paradigm advocates `agents' to perform local computations and exchange intermediate variables with other agents across edges of a communication network to solve the problem. In this paper, we consider three different grid optimization problems and cast them as examples of a constrained convex optimization program. In each problem setting, we adopt different power flow models, different notions of agents and different notions of the network over which these agents interact. In doing so, we view these disparate grid optimization problems as examples of a generic constrained convex optimization problem $\Pcal$ that facilitates unified algorithm development and analysis. We consider three different grid optimization problems:
\begin{itemize}[leftmargin=*]
    \item \emph{Multi-area optimal power flow  ($\Pcal_1$)} seeks to dispatch resources over an interconnected transmission network, parts of which are controlled by different system operators. The distributed algorithmic architecture bypasses the need for the system operators to share all relevant data from within their footprint with another system operator and yet seek to solve a joint optimal power flow problem through a distributed solution architecture.
    \item \emph{Coordination of distributed energy resources (DERs) in distribution grids ($\Pcal_2$)} is designed to optimize real and reactive power outputs from DERs at the grid-edge to minimize cost (dis-utility) of such a dispatch and possibly a network-wide objective such as frequency regulation. A distributed algorithm allows quick updates of optimization variables without the need to communicate with a central coordinator across the distribution grid.
    \item \emph{Transmission and distribution (T\&D) grid coordination ($\Pcal_3$)} seeks to dispatch assets across the transmission and distribution grids without the need to collect all information from the grid-edge and the bulk power systems at one location. The distributed solution architecture alleviates the transmission system operator's lack of visibility into utility-managed distribution networks.
\end{itemize}

These problems are nonconvex due to the nature of Kirchhoff's laws \cite{cain2012history}. In this paper, we \emph{convexify} them by considering power flow models that are suited to each problem. For $\Pcal_1$, we consider a linear power flow model for transmission networks motivated by the use of such models in wholesale market environments that facilitate inter-area coordination. For $\Pcal_2$, we consider a second-order cone programming (SOCP) based relaxation of the power flow equations in the distribution grids. The thoroughly-studied SOCP-based relaxation of power flow equations for distribution grids are often tight in practice (see \cite{Farivar2013,gan2015exact}). 
% That is, an optimal solution of the convex problem often yields a point feasible in the original nonconvex optimization problem. 
For $\Pcal_3$, we consider two different power flow models for the transmission and the distribution grids. For transmission, we choose a semidefinite programming (SDP) based relaxation of power flow equations, given its popularity to approach the AC optimal power flow problem \cite{lavaei2011zero,zhang2012geometry,bose2015quadratically}. For the distribution grids, we consider the linear distribution power flow model from \cite{Baran1989c}.


We view these distinct problems in power system operation through a unifying lens that allows us to study algorithm design in a unified framework. While many techniques apply to these problems, in this paper, we study \emph{distributed dual subgradient methods with averaging}, addressed recently in \cite{liang2019distributed}. At its core, this algorithm relies on dual decomposition that starts by separating the Lagrangian into agent-wise Lagrangian functions that each agent optimizes, given a dual iterate (see classical texts such as \cite{BertsekasTsitsiklis1989}). Such an update rule requires a central coordinator to manage the dual iterates. Distributed dual subgradient methods maintain \emph{local copies} of such multipliers and run a consensus-based distributed dual ascent on these local multipliers. Approximate primal solutions can be recovered from these dual solutions as in \cite{simonetto2016primal}, building on techniques in \cite{Nedic2009,gustavsson2015primal,ma2007recovery}; asymptotic guarantees on recovered primal sequences are known. In this paper, we study a distributed dual subgradient method, analyzed recently in \cite{liang2019distributed} that generalizes the centralized counterpart in \cite{nesterov2018dual}. For the fully distributed algorithm, with decaying step-sizes, the authors characterize a $\Ocal(\log T/\sqrt{T})$-bound on a metric that combines sub-optimality and constraint violation, while they argue a lower bound of $\Ocal(1/\sqrt{T})$. Our analysis closes the gap between these bounds, i.e., we sharpen the convergence rate to $\Ocal(1/\sqrt{T})$ with \emph{constant step-size}. 
% Our choice is motivated to avoid known pitfalls of diminishing step-sizes in practical applications (see \cite{simonetto2016primal}).


% Overall, we present a unified framework to study three different grid optimization problems, provide a sharper convergence rate for a recently-studied algorithm and share results from numerical experiments of the same algorithm for the three applications. 



{\color{blue} Concretely, our contributions are as follows.
\begin{itemize}[leftmargin=*]
    \item We provide an improved finite-time convergence result for distributed dual subgradient algorithm with averaging on $\Pcal$, compared to \cite{liang2019distributed}, and argue that it is order-optimal. 
    
    \item As will be clear from our literature survey, many prior works have developed algorithms for grid optimization problems $\Pcal_1, \Pcal_2, \Pcal_3$ with specific power flow models, few among which come with provable finite-time performance guarantees. Instead, we present these problems with multiple power flow models (suitable to each application), and reduce each to an instance of $\Pcal$. As a result, our algorithm for $\Pcal$ and its rate analysis  applies to all applications.
    
    \item Through the numerical example on $\Pcal_1$, we demonstrate how the averaging scheme stabilizes the last iterate, compared to classical dual subgradient methods, and circumvents the need for primal recovery. We also show that finite-time constraint violation of the algorithm is empirically better than its theoretical bound, that invites future analysis.
    
    \item Through examples of $\Pcal_2$, we show that our algorithm can track changing grid conditions for small networks. Tracking performance degrades with network size, where aggregation of nodes becomes vital for performance. 
    
    \item Using an example of $\Pcal_3$, we compare the empirical performance of our dual subgradient method with a naively adopted distributed acceleration scheme, and show how acceleration scheme fails to increase convergence speed. We argue that nonsmoothness of the dual function lies at the heart of this issue and elaborate on this in Appendix \ref{sec:dual_func}.
\end{itemize}
}

In Section \ref{sec:algorithm}, we present a generic constrained multi-agent convex optimization problem as $\Pcal$ and present our convergence result. Then, we reduce the application problems $\Pcal_1$, $\Pcal_2$ and $\Pcal_3$ as instances of $\Pcal$ in Sections \ref{sec:multi_area}, \ref{sec:DER_coord} and \ref{sec:TD_coordination}, respectively. For problem, we describe prior art, identify it as an instance of $\Pcal$ and document numerical results of running the algorithm from Section \ref{sec:algorithm}.


% Closest in spirit to this work is the survey in \cite{Molzahn2017} that provides an extensive review on distributed optimization techniques for optimal power flow (OPF) problems with various power flow models. The list of techniques include augmented Lagrangian decomposition, Karush-Kuhn-Tucker conditions-based approaches, gradient dynamics and dynamic programming methods with applications to voltage/frequency control. In contrast, we study an algorithm that was discovered after the survey was published, provide a sharper convergence guarantee for it and apply it to specific grid optimization problems with appropriate power flow models. 





%-----------------

\iffalse
\bose{Please move the prior work in respective sections.}
\subsection{Prior Work}
\bose{Put the prior works in the respective sections.}
A survey paper \cite{Molzahn2017} has presented an extensive review on the distributed optimization for OPF, and algorithms for online optimization and control of power system problems. In the first half of the paper, \cite{Molzahn2017} introduced various models for power flow equations including the DistFlow \cite{Baran1989c}, Linearized DistFlow \cite{Baran1989a,Baran1989b}, DC OPF, and the non-convex OPF problem together with its convex relaxations based on those models. 
 Afterward, \cite{Molzahn2017} summarizes distributed optimization techniques to solve OPF problems in the form of a collection of methods such as augmented Lagrangian decomposition, KKT conditions based approaches, gradient dynamics and dynamic programming methods. In the second half, \cite{Molzahn2017} surveyed various works on the optimization and control of optimal frequency control, optimal voltage control, and optimal wide-area control problems. Two sets of distributed optimization techniques were considered in \cite{Molzahn2017}: (i) augmented Lagrangian decomposition based; (ii) Karush-Kuhn-Tucker (KKT) necessary conditions based. 
%, while our current paper presents a unified framework to solve any optimization problem which can be written in the form of {\Pcal}. 

Next, another recent work \cite{TYang19} has been conducted on continuous-time and discrete-time distributed optimization approaches with particular attention on the optimal DER coordination problem. The main category of approaches considered in \cite{TYang19} is first-order approaches, although a few second-order methods was mentioned. However, the central focus for inter-agent communication graph in \cite{TYang19} is on undirected ones, which limits the class of communications between agents. In addition, the DER coordination problem in  \cite{TYang19} is simple, where no power flow constraints were investigated, and the power balance constraint is the only coupling constraint there. 


\subsubsection{For Tie-line Scheduling Problem} 
 


\subsubsection{For DER Coordination Problem} 
 

\subsubsection{For T\&D Coordination Problem} 


\fi

%Conventionally, grid optimization problems are solved by centralized algorithms, for instance the optimal power flow (OPF) problem is solved by independent system operators (ISOs) to derive an optimal power dispatch strategy that minimizes some generation cost functions. However, in modern power grids where lots of sensors, e.g., phase measurement unit (PMU), smart meters, or distributed energy resources, e.g., rooftop PV, storage systems, electric vehicles (EVs), controllable loads, etc., are highly integrated into the grid, the existing centralized algorithms face challenges on dealing with a huge amount of data to be processed and a very large number of devices to be communicated. This certainly poses significant problems on the computation and communication time as well as the security and resiliency of power grids. Therefore, distributed algorithms should be developed as an solution to the aforementioned challenges. 

%Employing Multi-Agent System (MAS) theory, distributed control and optimization algorithms can be derived for power grids where each agent can represent an individual bus or a portion of the grid. Distributed algorithms then provides advantages over classical centralized algorithms where each agent only needs to collect and process a limited amount of information on a part of the grid assigned to it, and communicate to a limited number of neighboring agents. Thus, the disadvantages of centralized algorithms on the communication and computation time, and their security  mentioned above can be improved with distributed algorithms. As a result, the data privacy , the algorithm scalability and speed can be significantly advanced with parallel and distributed computation in distributed algorithms. 


%In this paper, we cast a collection of grid optimization problems as examples of 




==> literature_review.tex <==
%!TEX root = MainDistOptPower.tex

\newpage

\textbf{Abstract}

This report mainly consists of two sections.
First, we provide some suggestions in showing the contributions and highlights of our work. Then we summarize all the papers shared by Prof. Hoa (not including the review and thesis). We evaluate each paper in the following six aspects.
\begin{enumerate}[leftmargin=*]
    \item Classification of the algorithm.
    \item Scenario settings. (network model and special elements.)
    \item The special treatment for applying the algorithm into the scenario.
    \item Implementation briefs of the algorithm.
    \item Initialization, stopping criteria, case studies.
    \item Theoretical analysis of the algorithm.
\end{enumerate}

\textbf{Abbreviations}

Abbreviations for the Journal and Conference papers
\begin{itemize}[leftmargin=*]
    \item Journal
    \begin{itemize}[leftmargin=*]
    \item TPS: IEEE Transactions on Power Systems,
    \item TAC: IEEE Transactions on Automatic Control,
    \item TSE: IEEE Transactions on Sustainable Energy,
    \item TASE: IEEE Transactions on Automation Science and Engineering,
    \item TITS: IEEE Transactions on Intelligent Transportation Systems, 
    \item EPSR: Electric Power Systems Research,
    \item AE: Applied Energy,
    \item Energy,
    \item ECM: Energy Conversion and Management
    \item EURASIP: EURASIP Journal on Advances in Signal Processing,
    \item SEGN: Sustainable Energy, Grids and Networks,
    \item arXiv
    \end{itemize}
    \item Conference
    \begin{itemize}[leftmargin=*]
    \item PESGM: IEEE Power \& Energy Society, General Meeting
    \item PowerTech: IEEE PowerTech
    \item SGC: IEEE International Conference on Smart Grid Communications
    \end{itemize}
\end{itemize}
    

\textbf{Contributions \& Highlights}

\textbf{Contributions}

We summarize the contribution of our work in terms of high transferability, convergence guarantees, and generalization.
\begin{enumerate}[leftmargin=*]
    \item High transferability. In terms of algorithm development, many algorithms are tailored for specific scenarios. Among the three, MAOPF is classic which enjoys abundant researches in early times. DER and T\&D problems are new with relatively few studies. In our work, we unified three scenarios, which show the generic of the proposed method and provide guidance in how to adapt the methods from early work of MAOPF into DER and T\&D.
    \item Convergence guarantees. Early work tailored for power systems usually does not ensure convergence. Some of them may even not converge at all, which may be risky for power system operations. In our work, we verified the effectiveness of the proposed method with simulations and theoretical convergence analysis.
    \item Generalization. We choose three scenarios with increasing model complexity, i.e., LP/SOCP/SDP. Thus, our method can adapt much suitable approximation and many convex relaxation techniques of the network model. It is also ideal for more customized operation demands. 
\end{enumerate}

\textbf{Highlights}

\begin{enumerate}[leftmargin=*]
    \item Many Lagrangian relaxation-based methods in power systems do not emphasize the feasibility issue. Only the work in \cite{papadaskalopoulosDecentralizedCoordinationMicrogrids2014} proposes an empirical rule which sacrifices the optimality.
    \item A fast practical convergence on a 8-area 767-bus system using modified dual decomposition is illstratied in \cite{LaiXXZK2015}.
    \item Many DER problems adopt primal decomposition by using a penalty-based formulation without involving dual values. The work in \cite{cherukuriDistributedCoordinationDERs2018a} exchanges primal values using a {\bf dynamic averaging consensus} update. The drawback is that the optimal primal solutions are known to all agents when reaching a consensus.
    \item The consensus update gets interested in the power system from DER coordination. For example \cite{dominguez-garciaCoordinationControlDistributed2010} reach a consensus on power balance with some empirical allocation rules. To realize an optimal dispatch, "Consensus + Innovation" has introduced the sub-gradient of local costs to update, see \cite{wuDistributedOptimalCoordination2017a} for example. They are like early simplified versions of our work.
    \item We admit there are many other new methods, but they do not directly relate to power system operations. It is beyond the scope of the review in this round.
\end{enumerate}

\textbf{Research work shared from Prof. Hoa}

\haitian{Here, we differentiated primal or dual decomposition by updating primal or dual variables in the second stage. Maybe some primal decomposition approach also form Lagrangian function in the first stage, see \cite{luFullyDecentralizedOptimal2018a} for example.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{MAOPF}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{MAOPF-2003-Dual DD/OCD([TPS], Bakirtzis, A.G. \& Biskas, P.N.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{bakirtzisDecentralizedSolutionDCOPF2003a} was published in 2003. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is classic dual decomposition. It is a coordinated approach.
    \item The application scenario is MAOPF with a DC network model, considering no particular elements.
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment introduces copies of boundary voltages, and tie-line flows to reform coupling constraints. Thus, boundary energy balance becomes a local constraint.
    \item Implementation briefs. The algorithm first solves a local Lagrangian problem. And then, the coordinator updates dual variables by exchanging neighbors' phase angles and tie-line flows.
    \item The algorithm is synchronous, specified cold start for multipliers. The paper measures convergence by the mismatch of the consistency constraints. The test deploys a 5-area 583-bus system, showing a fixed 25 iterations.
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2017-Dual DD/OCD([PowerTech], Halilbasic, Lejla \& Chatzivasileiadis, Spyros \& Pinson, Pierre)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{halilbasicCoordinatingFlexibilityUncertainty2017} was published in 2017. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is standard OCD. It is a coordinated approach.
    \item The application scenario is MAOPF with a DC network model, considering RES uncertainties, DC lines, and reserve.
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment introduces tie-line power flow as ancillary variables to reform coupling constraints.
    \item Implementation briefs. The algorithm first solves a local Lagrangian problem. And then, the coordinator updates dual variables by exchanging neighbors' dual variables and phase angles (tie-line flows).
    \item The algorithm is asynchronous, with specifying initial values. The paper measures convergence by the mismatch of the tie-line flows. The test deploys a 3-area RTS-96 system, showing convergence after 27 iterations.
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2007-Dual DD/OCD([PowerTech], Arnold, Michele \& Knopfli, Selina \& Andersson, Goran)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{arnoldImprovementOPFDecomposition2007} was published in 2007 and proposed two algorithms that adopted Lagrangian relaxation and augmented LR of dual decomposition. The specific methods taken are standard dual decomposition and APP. They are both coordinated approaches.
    \item The application scenario is MAOPF with an AC network model, considering no particular elements.
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment introduces copies of coupling variables. Besides, a two-stage structure can be empirically assigned to satisfy customized needs, with certain coupling constraints fixed in the second stage.
    \item Implementation briefs. For standard dual decomposition, the dual variables conduct a sub-gradient update from the mismatch of the duplicated variables. For APP, the updates are similar to the first with penalty terms.
    \item The algorithm is synchronous, without specifying initial values. The paper measures convergence by the mismatch of variables in two consecutive steps. The test deploys a 2-area 39-bus system, showing convergence after 258 iterations.
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides no convergence guarantees. Besides, there are several strategies with merely empirical convergence.
\end{enumerate}

\textbf{MAOPF-2013-Dual DD/OCD([TPS], Ahmadi-Khatir, Ali \& Conejo, Antonio J. \& Cherkaoui, Rachid)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{ahmadi-khatirMultiAreaEnergyReserve2013a} was published in 2013. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is standard OCD. It is a coordinated approach, and a derivative work to \cite{Nogales2003ADM}.
    \item The application scenario is MAOPF with a DC network model, considering RES, reserve, and equipment failures. 
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment is introducing tie-line power flow as ancillary variables to reform coupling constraints.
    \item Implementation briefs. Each agent solves a local Lagrangian problem. And then, the update uses exchanged neighbor's phase angles and dual variables to realize a local dual update.
    \item The algorithm is synchronous, specified with feasible primal and dual initial values. The paper measures convergence by the mismatch of the dual values in 2 consecutive iterations. The test deploys a 3-area Reliability Test System RTS(72-bus) system with 24 planning horizons, showing convergence after 2410 [seconds].
    \item The algorithm is a first-order method with empirical asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2014-Dual DD/OCD([PESGM], Lai, Xiaowen \& Xia, Qing \& Xie, Le)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{laiInterareaPowerExchange2014} was published in 2014. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is modified OCD. It is a coordinated approach and an early work of \cite{LaiXXZK2015}.
\end{enumerate}

\textbf{MAOPF-2015-Dual DD/OCD([TPS], Lai, Xiaowen \& Xie, Le \& Xia, Qing \& Zhong, Haiwang \& Kang, Chongqing)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{LaiXXZK2015} was published in 2015. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is dual decomposition. It is a coordinated approach and a derivative work of \cite{bakirtzisDecentralizedSolutionDCOPF2003a}.
    \item The application scenario is MAOPF with a DC network model, considering no particular elements.
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment introduces tie-line power flow as ancillary variables to reform coupling constraints.
    \item Implementation briefs. The algorithm first solves a local Lagrangian problem. And then, the coordinator updates dual variables by exchanging neighbors' dual variables and phase angles (tie-line flows). Moreover, the paper proposes a linear relation for dual update based on sensitivity, called "dynamic update."
    \item The algorithm is synchronous, specified with cold start for multipliers, zero initial tie-line flows. The paper measures convergence by the mismatch of the tie-line flows. The test deploys an 8-area 767-bus system, showing convergence after 579 iterations.
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2017-Dual Non-iterative([TPS], Ji, Yuting \& Zheng, Tongxin \& Tong, Lang)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{jiStochasticInterchangeScheduling2017} was published in 2017. It adopts dual decomposition. The specific method taken is finding the equilibrium of supply and demand functions. It is a coordinated approach.
    \item The application scenario is MAOPF with a DC network model (shift factor-based), considering uncertainty. 
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment is introducing a single proxy bus as net interchange $q$ to decompose the system.
    \item Implementation briefs. Each region submits an (expected) LMP curve about its proxy bus w.r.t. $q$. And then, the coordinated update is done by finding the equilibrium (intersection) among the (expected) LMP. Thus, there is no need for iteration.
    \item The test deploys a 2-area 118-bus and a 3-area 30-bus system, respectively.
    \item There is no need to illustrate convergence. However, note that the final solutions may be suboptimal because introducing the proxy bus approximates the original DCOPF.
\end{enumerate}

\textbf{MAOPF-2015-Dual ADMM([EURASIP], Erseghe, Tomaso)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{ersegheDistributedApproachOPF2015} was published in 2015. It adopts augmented Lagrangian relaxation of dual decomposition. The specific method taken is ADMM with an adaptive penalty. It is a coordinated approach.
    \item The application scenario is MAOPF with an AC network model, considering no particular elements.
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment introduces copies of boundary voltages, and tie-line flows to reform coupling constraints.
    \item Implementation briefs. The algorithm first solves a local augmented Lagrangian problem. And then, the coordinator updates dual variables and the penalty parameters by exchanging neighbors' voltages and penalties, respectively.
    \item The algorithm is synchronous, specified cold start for multipliers, 1.0 p.u. for initial primal values. Moreover, there are artificial bounds on the dual variables. The paper measures convergence by the mismatch of the consistency constraints. The test deploys a 69-area 300-bus system, showing convergence after 216 iterations.
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2016-Dual ADMM([arXiv], Guo, Junyao \& Hug, Gabriela \& Tonguz, Ozan)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{guoEnablingDistributedOptimization2016} was published in 2016. It adopts augmented Lagrangian relaxation of dual decomposition. The specific method taken is ADMM with \haitian{system partition technique}. It is a coordinated approach and a derivative work of \cite{ersegheDistributedApproachOPF2015}.
    \item The application scenario is MAOPF with an AC network model, considering no particular elements.
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment introduces copies of boundary voltages, and tie-line flows to reform coupling constraints. The paper uses spectral clustering of an affinity matrix of the entire system, with the K-means method as the last step to partition the system into $K$ regions.
    \item Implementation briefs. The algorithm first solves a local augmented Lagrangian problem. And then, the coordinator updates dual variables and the penalty parameters by exchanging neighbors' voltages and penalties, respectively.
    \item The algorithm is synchronous, specified with cold start for multipliers, 1.0 p.u. for initial primal values. The paper measures convergence by the mismatch of the consistency constraints. The test deploys a 90-region Polish 2383-bus system, showing convergence after 300 iterations.
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2013-Dual ADMM([ECM], Doostizadeh, Meysam \& Aminifar, Farrokh \& Lesani, Hamid \& Ghasemi, Hassan)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{doostizadehMultiareaMarketClearing2016} was published in 2016. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is parallel ADMM. It is a coordinated approach.
    \item The application scenario is MAOPF with a DC network model, considering RES. 
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment is introducing copies of boundary phase angles to reform coupling constraints.
    \item Implementation briefs. Each agent solves a local augmented Lagrangian problem. And then, the coordinate update becomes a consensus update for phase angles with uniform weight rules and then a local dual update (i.e., Consensus ADMM).
    \item The algorithm is synchronous, specified cold start initialization for consensus primal and dual values. For comparison, there is also a classic asynchronous consensus ADMM. The paper measures convergence by primal and dual residuals. The test deploys a 3-area 118-bus system, which has not shown any iterations.
    \item The algorithm is a first-order method with empirical asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2017-Dual ADMM and C\&CG([TPS], Li, Zhigang \& Wu, Wenchuan \& Shahidehpour, Mohammad \& Zhang, Boming)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{liDecentralizedContingencyConstrainedTieLine2017} was published in 2017. It adopts dual decomposition. The specific method taken is ADMM and column and constraints generation (C\&CG). It is a coordinated approach and a derivative work of \cite{liAdaptiveRobustTieLine2016a}.
    \item The application scenario is MAOPF with a DC network model, considering the multi-time period, RES, reserve, robust optimization, and $n-k$ contingency. 
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment is to introduce copies of boundary phase angles such that the master problem of C\&CG becomes decomposable. There is also a robust version of the problem, which uses KKT reformulation, and is penalized by the big-M method. The final robust counterpart local problem is binary MIP.
    \item Implementation briefs. Each agent conducts a local C\&CG procedure. And then, the master problem has decomposed into local dual updates using consensus ADMM, where the averaging part is the boundary phase angles by a uniform weight rule.
    \item The algorithm is synchronous, specified with initial solutions to the C\&CG master problem (warm start). There is also a scenario update technique to improve computational efficiency. The paper measures convergence by the primal and dual residuals of consensus ADMM. The test deploys a 4-area 1441-bus system with 24 planning horizons, showing convergence after 307 iterations for $N-2$ contingency.
    \item The algorithm is a first-order method with empirical asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2015-Dual ADMM and C\&CG([TSE], Li, Zhigang \& Zeng, Bo \& Zhang, Boming \& Zheng, Weiye)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{liDecentralizedMultiareaRobust2015} was published in 2015. It adopts dual decomposition. The specific method taken is ADMM and column and constraints generation (C\&CG). It is a coordinated approach and an early work to \cite{liDecentralizedContingencyConstrainedTieLine2017}.
    \item The application scenario is MAOPF with a DC network model, considering RES and unit commitment. 
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment is to introduce copies of boundary phase angles such that the master problem of C\&CG becomes decomposable. There is also a robust version of the problem, which uses KKT reformulation, and is penalized by the big-M method. The final robust counterpart local problem is binary MIP.
    \item Implementation briefs. Each agent conducts a local C\&CG procedure. And then, the master problem has decomposed into local dual updates using consensus ADMM, where the averaging part is the boundary phase angles by a uniform weight rule.
    \item The algorithm is synchronous, specified with initial solutions to the C\&CG master problem (warm start). There is also a scenario update technique to improve computational efficiency. The paper measures convergence by the primal and dual residuals of consensus ADMM. The test deploys a 3-area 118-bus system with 24 planning horizons, showing convergence after 437 [seconds].
    \item The algorithm is a first-order method with empirical asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2016-Primal C\&CG([TPS], Li, Zhigang \& Wu, Wenchuan \& Shahidehpour, Mohammad \& Zhang, Boming)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{liAdaptiveRobustTieLine2016a} was published in 2016. It adopts primal decomposition. The specific method taken is column and constraints generation (C\&CG). It is a coordinated approach, and a derivative work of \cite{zengSolvingTwostageRobust2013}.
    \item The application scenario is MAOPF with a DC network model (shift factor-based), considering the multi-time period, RES, and robust optimization. 
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment is to use network equivalence to calculate boundary power injection.
    \item Implementation briefs. Each agent solves a C\&CG sub-problem. And then, the coordinate update is to solve a Benders type master problem (MP). There are appended local variables to MP from binding constraints (column generation) and constraints from optimal solutions (cut generation). Local problem submits cuts purely involving primal variables.
    \item The algorithm is synchronous, specified with initial solutions to the C\&CG master problem (warm start). The paper measures convergence by the Benders' upper and lower bound. The test deploys a 4-area 1441-bus system with 24 planning horizons, showing convergence after 838 iterations for $N-2$ contingency.
    \item The algorithm is a first-order method with finite convergence for LP, asymptotic convergence for QP. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2014-Primal coordinated dispatch algorithm([COR], Baldick, Ross \& Chatterjee, Dhiman)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{baldickCoordinatedDispatchRegional2014a} was published in 2014. It adopts primal decomposition. The specific method taken is the coordinated dispatch algorithm. It is a coordinated approach.
    \item The application scenario is MAOPF with a DC network model (shift factor-based), considering each branch's exogenous determined loop flow capacity.
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment introduces two ancillary variables, i.e., 1) regional interchange (RI) used to decompose power balance, 2) commercial flow allocation (CFA) used to decompose the portion of the branch flow. (CFA indicates the portion of regional power flow that can transfer at a specific branch.)
    \item Implementation briefs. Each agent solves a local problem with given primal variables RI and CFA. And then, RI and CFA conduct a coordinated update using empirical relation to LMP with some weight coefficients.
    \item The algorithm is synchronous, specified with a feasible warm start. The paper does not measure convergence. The test deploys a 17-bus system, showing 25 fixed iterations.
    \item The algorithm is a first-order method with empirical primal convergence. The paper provides no convergence guarantees. The results may be suboptimal.
\end{enumerate}

\textbf{MAOPF-2014-Primal MED([TPS], Zhao, Feng \& Litvinov, Eugene \& Zheng, Tongxin)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{ZhaoLZ2014} was published in 2014. It adopts primal decomposition. The specific method taken is Marginal Equivalent Decomposition (MED). It is a coordinated approach. 
    \item The application scenario is MAOPF with a DC network model, considering no particular elements.
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment introduces slacks to equality and inequality constraints.
    \item Implementation briefs. The coordinator updates by exchanging binding constraints and variables related to simplex pivoting after each agent solve its local problem.
    \item The algorithm is asynchronous, without specifying initial values. The paper measures convergence by the improvement of the reduced cost to all sub-problems. The test deploys a 2-area 13-bus system, showing convergence after five iterations, and a New England–New York system with fixed iterations.
    \item The algorithm is a first-order method with empirical finite step convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2015-Primal Model Predictive Control([TPS], Kahl, Matthias \& Freye, Claudius \& Leibfried, Thomas)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{kahlCooperativeMultiAreaOptimization2015} was published in 2015. It adopts primal decomposition. The specific method taken is model predictive control (MPC). It is a coordinated approach.
    \item The application scenario is MAOPF with a DC network model, considering the multi-time period, RES, storage devices, and re-dispatch.
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment is to use external power generation for each area to decompose the system.
    \item Implementation briefs. The coordinate update is to assign system state (State of Charge), all local agents adjust local and external generation correspondingly to meet power balance.
    \item The algorithm is synchronous, specified with feasible initial primal solutions by solving an ancillary optimization (warm start). The paper measures convergence by the cost difference calculated by respective areas. The test deploys a 6-area 118-bus system, showing no convergence results.
    \item The algorithm is a first-order method with suboptimal solutions. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2018-Primal Coordinate Descent([TPS], Ji, Yuting \& Tong, Lang)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{jiMultiAreaInterchangeScheduling2018} was published in 2018. It adopts primal decomposition. The specific method taken is Coordinate Descent. It is a coordinated approach.
    \item The application scenario is MAOPF with a DC network model, considering the multi-time period and load uncertainty.
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment introduces one ancillary variable, i.e., regional interchange ($q$), to decompose power balance. The paper adopts an approximate mapping relation between $q$ and the LMP to form the supply and demand function.
    \item Implementation briefs. In each iteration, regional $i^{\text{th}}$ interchange will be updated sequentially by intersecting the expected supply and demand functions.
    \item The algorithm is asynchronous, specified with feasible initial primal solutions. The paper measures convergence by the regional interchange ($q$) does not change significantly in two consecutive iterations. The test deploys a 3-area 118-bus system, showing convergence after 838 iterations.
    \item The algorithm is a first-order method with empirical primal convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{MAOPF-2018-Primal Distributed IPM([TPS], Lu, Wentian \& Liu, Mingbo \& Lin, Shunjiang \& Li, Licheng)}

\haitian{One difference between this method and OCD-C is that this method adopts an exact update while OCD-C is an approximate update by neglecting off-diagonal terms.}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{luFullyDecentralizedOptimal2018a} was published in 2018. It adopts primal decomposition. The specific method taken is Interior Point Method (IPM) and \haitian{parametric programming}. It is a coordinated approach.
    \item The application scenario is MAOPF with an AC network model, considering no particular elements.
    \item The algorithm solves the scenario in a \haitian{distributed} fashion. The special treatment introduces copies, i.e., voltages and phase angles, and augments all the constraints with slack variables. Thus, the KKT condition becomes a linear system, where centralized IPM can solve it using Newton-Raphson iteration. Furthermore, the information passes to each agent one-by-one to realize decentralization (gossips).
    \item Implementation briefs. The N-R iteration solves in two-stage. First, the KKT system reformulates into a parametric QP in each iteration, where all the voltages and phase angles are parameters. The local primal and dual variables are decision variables. And then, the boundary information conducts an update according to the sum of the mapping value function. 
    \item The algorithm is asynchronous due to gossips, specified with cold start for multipliers, 1.0 p.u. for voltage magnitudes, and all zeros for phase angles. The paper measures convergence by the complementary gap of the IPM. The test deploys a 4-area 6056-bus system, showing convergence after 81 iterations.
    \item The algorithm is a first-order method with the same convergence to centralized IPM. The paper provides no convergence guarantees.
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{DER}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{DER-2014-Centralized Price incentive([TPS], Rahimiyan, Morteza \& Baringo, Luis \& Conejo, Antonio J.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{rahimiyanEnergyManagementCluster2014} was published in 2014. The specific method taken is a price incentive-based algorithm. It is a centralized approach.
    \item The application scenario is DER with a linear network model to maximize demand utility, considering demand response, multi-time period, battery storage, virtual power plant, and RES uncertainties using robust optimization techniques.
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment generates confidence intervals of price and wind uncertainties using ARIMA and AR, respectively. Furthermore, reform the initial problem with the confidence intervals into a robust counterpart LP problem. 
    \item Implementation briefs. The coordinator schedules the generation plan for DR or RES with a given price from predicted at current time $t$. DR or RES follow these dispatch orders. The coordinator then predicts a new price at time $t + 1$ until the end of the day.
    \item The algorithm has not specified initial values. The test deploys multiple DERs on a 5-bus network. There is no point in showing convergence. Nevertheless, the authors provide various operation modes from a practical view.
    \item The algorithm is not quite like a distributed algorithm. A coordinator solves the centralized problem. And then, all DR and RES follow dispatch orders to realize a distributed structure.
\end{enumerate}

\textbf{DER-2010-Primal Consensus([SGC], Dominguez-Garcia, Alejandro D. \& Hadjicostis, Christoforos N.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{dominguez-garciaCoordinationControlDistributed2010} was published in 2010. It adopts primal decomposition. The specific method taken is a consensus update. It is a distributed approach.
    \item The application scenario is DER without a network model, considering no particular elements.
    \item The algorithm solves the scenario in a distributed fashion. The special treatment is to set one agent as a leader such that the final consensus is to let all agents collectively satisfy the demand demanded from the leader.
    \item Implementation briefs. The method is a pure consensus without gradient information involved. For an unconstrained case, each agent conducts a consensus update. For the constrained case with a capacity limit, the paper proposes different splitting strategies to allocate the generation capacity for each DER. When reaching a consensus, how much generation each node contributes depends on both the communication matrix (row \& column stochastic) and the splitting strategy. 
    \item The algorithm is synchronous, specified with zero initial value and unit demand. The test deploys 5 DERs on a 5-bus system, showing a fixed 60 iterations.
    \item The algorithm is not for optimization.
\end{enumerate}

\textbf{DER-2018-Primal Practical([TSG], Bhattarai, Bishnu P. \& de Cerio Mendaza, Iker Diaz \& Myers, Kurt S. \& Bak-Jensen, Birgitte \& Paudyal, Sumit)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{bhattaraiOptimumAggregationControl2018} was published in 2018. It adopts primal decomposition. The specific method taken is a control-based algorithm. It is a coordinated approach.
    \item The application scenario is DER without a network model, considering optimal demand aggregation based on spatial distance, demand response, and electricity market.
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment is to \haitian{find clusters to reduce the network using spatial distance.} Then, the DSO can only interact with the clusters.
    \item Implementation briefs. The central coordinator monitors the system's voltage, power consumption, and grid violations. If deviations or violations occur, the coordinator regulates the aggregators' dispatch level, and all the DERs respond accordingly. 
    \item The algorithm deploys on a real-world distribution network located in the southeast of Denmark and owned by Danish DSO SEAS-NVE. This algorithm is a pretty practical approach, and there is no convergence analysis found.
\end{enumerate}

\textbf{DER-2018-Primal Extremum Seeking([TPS], Arnold, Daniel B. \& Sankur, Michael D. \&  Negrete-Pincetic, Matias \& Callaway, Duncan S.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{arnoldModelFreeOptimalCoordination2018a} was published in 2018. It adopts penalty-based primal decomposition. The specific method taken is Extremum Seeking. It is a coordinated approach.
    \item The application scenario is DER with a DistFlow model (nonconvex) using local second-order Taylor expansion, considering no particular elements.
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment uses penalty to reform all network constraints into the objective function. Furthermore, there is a feedback control loop for describing the detailed implementation of the algorithm, which contributes to model-free coordination.
    \item Implementation briefs. Each local DER agent updates controllable active and reactive power measurements using the Extremum Seeking control loop in the corresponding two dimensions. The coordinator captures the mapping from real and reactive power injected into the system to measurements observed to construct and then built a penalty-based function using local Taylor expansion. The control feedback returned to all local agents using a high pass (washout) filter split into two channels. \haitian{I think this step is similar to gradient update.}
    \item The algorithm has not specified initial values. The test deploys 4 DERs on a 37-bus network. There is no result showing convergence. Nevertheless, the authors provide detailed guidance in selecting parameters of the algorithm.
    \item The algorithm is a first-order method with \haitian{local} asymptotic convergence. The paper provides some local convergence guarantees. However, there is no apparent convergence rate.
\end{enumerate}

\textbf{DER-2016-Primal Game \& Consensus([TAC], Gharesifard, Bahman \& Basar, Tamer \& {Dominguez-Garcia}, Alejandro D.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{gharesifardPriceBasedCoordinatedAggregation2016} was published in 2016. It adopts a consensus update of primal decomposition. The specific method taken is concave game formulation \& consensus update. It is a distributed approach.
    \item The application scenario is DER without a network model, considering DER's utility, aggregator's pricing incentive, and continuous time.
    \item The algorithm solves the scenario in a distributed fashion. The special treatment is to cast the problem as a concave game finding unique Nash equilibrium under certain conditions.
    \item Implementation briefs. Local primal variables (estimates) are first updated using local gradients. Then all estimates conduct a consensus update. These two steps repeat recursively.
    \item The algorithm has not specified initial values. The test deploys 6 DERs communicated over an undirected graph, showing convergence after a fixed 30 [seconds].
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides convergence guarantees. However, there is no apparent convergence rate.
\end{enumerate}

\textbf{DER-2018-Primal Dynamic Average Consensus([TAC], Cherukuri, Ashish \& Cort{\'e}s, Jorge)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{cherukuriDistributedCoordinationDERs2018a} was published in 2018. It adopts a consensus update of primal decomposition. The specific method taken is exact penalty function \& dynamic average consensus. It is a distributed approach.
    \item The application scenario is DER without a network model, with the consideration of storage.
    \item The algorithm solves the scenario in a distributed fashion. The special treatment is to reform all inequalities into the objective functions using the exact penalty approach. The reformed problem has only one equality constraint for energy balance.
    \item The implementation briefs as local primal variables (estimates) are first updated using local and Laplacian gradients, then a consensus update for all estimates with dynamic averaging. These two steps repeat recursively until all the primal variables reach a consensus. \haitian{All the primal variables are known to all agents after converging.}
    \item The algorithm has not specified initial values. The test deploys 6 DERs communicated over a directed ring with six planning horizons, showing convergence after a fixed 300 [seconds].
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides convergence guarantees based on bounds of algorithm parameters, summarizing in Theorem 4.4. However, there is no apparent convergence rate.
\end{enumerate}

\textbf{DER-2017-Dual Consensus + Innovation([EPSR], Wu, Di \& Lian, Jianming \& Sun, Yannan \& Yang, Tao \& Hansen, Jacob)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{wuHierarchicalControlFramework2017} was published in 2017. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is "Consensus + Innovation." It is a coordinated approach.
    \item The application scenario is DER without a network model, considering demand response (DR). The scope of this paper is not to propose a new algorithm but to implement the hierarchical control structure from a practical view.
    \item The algorithm solves the scenario in a coordinated fashion. There is no special treatment.
    \item Implementation briefs. Local primal variables are first updated using local Lagrangian gradients with given dual variables. Then the local dual estimates are updated using local primal variables. Finally, all estimates conduct a consensus update by a coordinator. These three steps repeat recursively.
    \item The algorithm initializes with a cold start for dual variables, and the generation output the solution w.r.t to the initial dual values. The update is synchronous. The paper measures convergence by the mismatch of the dual values in 2 consecutive iterations. The test deploys an IEEE 123-bus system with three aggregators.
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{DER-2017-Dual Consensus + Innovation (Gradient)([TASE], Wu, Di \& Yang, Tao \& Stoorvogel, Anton A. \& Stoustrup, Jakob)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{wuDistributedOptimalCoordination2017a} was published in 2017. It adopts a consensus update of primal decomposition. The specific method taken is consensus update. It is a distributed approach.
    \item The application scenario is DER without a network model, considering storage.
    \item The algorithm solves the scenario in a distributed fashion. The special treatment is to convert the nonconvex state-of-charge using convex equivalency. (Non-convexity is due to the logical constraint for charging.)
    \item Implementation briefs. Local primal variables are first updated using local Lagrangian functions with given dual values. Then each agent updates dual values using local gradient and a consensus exchange of other dual estimates. These two steps repeat recursively.
    \item The algorithm has not specified initial values. The test deploys 4 DERs and two storage on a 6-bus network communicated over an undirected graph same as the physical topology. There is no result showing convergence.
    \item The algorithm is a first-order method with asymptotic convergence. The paper provides convergence guarantees. However, there is no apparent convergence rate.
\end{enumerate}
\bose{Does \cite{wuDistributedOptimalCoordination2017a} have a network or it does not?}


\textbf{DER-2017-Dual DD([AE], Wang, Jianxiao \& Zhong, Haiwang \& Lai, Xiaowen \& Xia, Qing \& Shu, Chang \& Kang, Chongqing)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{wangDistributedRealtimeDemand2017} was published in 2017. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is modified dual decomposition. It is a coordinated approach.
    \item The application scenario is DER without a network model, considering day-ahead dispatch and demand response (DR). 
    \item The algorithm solves the scenario in a coordinated fashion. There is no special treatment.
    \item Implementation briefs. Local consumers submit demand (decision variables), the coordinator (load-serving entity) returns coupling dual variables (congestion price) by solving a dual optimization (Lagrangian Multiplier Optimal Selection, LMOS). The dual problem forms the problem using (parametric mapping of) sensitivity analysis of local problem w.r.t congestion price.
    \item The algorithm is synchronous, which has not specified initial values. The paper measures convergence by the mismatch of the dual values in 2 consecutive iterations. The test deploys 100 consumers with twelve planning horizons, which has met the criteria in 110 iterations.
    \item The algorithm is a first-order method with empirical asymptotic convergence. The paper provides no convergence guarantees.
\end{enumerate}

\textbf{DER-2016-Dual Price incentive([TPS], Karfopoulos, Evangelos L. \& Hatziargyriou, Nikos D.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{karfopoulosDistributedCoordinationElectric2016} was published in 2016. It adopts dual decomposition. The specific method taken is a price incentive-based algorithm. It is a coordinated approach.
    \item The application scenario is DER without a network model, considering battery storage and EV (V2G).
    \item The algorithm solves the scenario in a coordinated fashion. There is no special treatment.
    \item Implementation briefs. Each local DER agent schedules a local generation plan with a given price from the coordinator. The coordinator collects all the generations and updates the price according to the gradient to minimize network load variance.
    \item The algorithm has not specified initial values. The test deploys multiple DERs on a realistic rural MV distribution network. There is no result showing convergence. Nevertheless, the authors provide various operation modes from a practical view.
    \item The algorithm is a first-order method with empirical convergence. However, the paper provides no convergence guarantees and convergence rates.
\end{enumerate}

\textbf{DER-2014-Dual DD([TSE], Papadaskalopoulos, Dimitrios \& Pudjianto, Danny \& Strbac, Goran)}


\begin{enumerate}[leftmargin=*]
    \item The paper \cite{papadaskalopoulosDecentralizedCoordinationMicrogrids2014} was published in 2014. It adopts Lagrangian relaxation of dual decomposition. The specific method taken is a modified dual decomposition. It is a coordinated approach.
    \item The application scenario is DER without a network model, considering energy storage and demand response. DR, ES, and EV want to arbitrage from LMP difference, while microgrid market operator (MGMO) wants to maximize congestion surplus (social welfare).
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment is \haitian{a practical way of recovering the feasibility of LR problems.} The results are suboptimal.
    \item Implementation briefs. Each local agent (EV, ES, DR, MGMO) optimizes local Lagrangian problems with given active \& reactive price for energy balance. The coordinator then updates the dual variables using a sub-gradient search. If the energy balance cannot be satisfied, all local agents will modify generation bounds artificially and resolve the local problem. 
    \item The algorithm is synchronous, specified with near-optimal multipliers. The paper measures convergence by power imbalance. The test deploys multiple DERs on a 17-bus system, showing convergence after 47 iterations.
    \item The algorithm is a first-order method with suboptimal solutions due to feasibility recovery.
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{T\&D}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{T\&D-2017-Primal Benders([AE], Yuan, Zhao \& Hesamzadeh, Mohammad Reza)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{ZYuan17} was published in 2017. It adopts primal decomposition. The specific method taken is Benders decomposition. It is a coordinated approach.
    \item The application scenario is T\&D with a SOCP relaxation for TSO and DSO network, considering reserve. 
    \item The algorithm solves the scenario in a coordinated fashion. The special treatment for TSO is to introduce power generation requirements (branch flow at T\&D interface) to decompose the system.
    \item Implementation briefs. Each local agent (DSO) submits Benders Cut. The coordinator (TSO) updates branch flow at the T\&D interface.
    \item The algorithm has not specified initial values. The update is synchronous. The convergence is measured by the Benders' upper and lower bound. The test deploys a 3-area system with one 14-bus TSO and two 13-bus DSO networks, showing convergence after three iterations, and a 390-bus practical network under various load conditions.
    \item The algorithm is a first-order method with finite convergence for LP, asymptotic convergence for QP. The paper provides no convergence guarantees.
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Others}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{OPF-2013([TPS], Jabr, Rabih A.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{jabrAdjustableRobustOPF2013} was published in 2013. It is a centralized approach to solve an affine adjustable robust optimization (AARO-OPF) problem. 
\end{enumerate}

\textbf{DER Planning-2018([TITS], Calvillo, Christian F. \& Sanchez-Miralles, Alvaro \& Villar, Jose)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{calvilloSynergiesElectricUrban2018} was published in 2018. It is a coordinated approach to solving a DER long-term planning problem.
    \item The application scenario is DER without a network model, considering battery, EV station investments, energy storage, metro, and energy price.
    \item The paper builds an LP model to trade off multi-objectives. The main contribution is to propose a  detailed integrated model.
\end{enumerate}

\textbf{DER-2016-Centralized([TPS], Yang, Fang \& Li, Zhao)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{yangImproveDistributionSystem2016} was published in 2016. It is a centralized approach.
    \item The application scenario is DER with a linear network model to loss reduction (optimal var flow) and voltage control, considering a detailed multiphase model.
    \item The algorithm solves the scenario in a centralized fashion. The main contribution of this work is modeling. Moreover, the authors verified the proposed loss reduction approach on nine practical distribution utility circuits.
\end{enumerate}

\textbf{DER-2017([Energy], Cardoso, G. \& Stadler, M. \& Mashayekh, S. \& Hartvigsson, E.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{cardosoImpactAncillaryServices2017} was published in 2017. It is a centralized approach to the DER expansion problem, considering ancillary services, such as frequency control, spinning, and non-spinning reserve.
\end{enumerate}

\textbf{DER-2015([EPSR], Alharbi, Walied \& Raahemifar, Kaamran)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{alharbiProbabilisticCoordinationMicrogrid2015} was published in 2015. It is a centralized approach to solving a DER coordination problem.
    \item The application scenario is DER without a network model, considering energy storage system(ESS), RES (controllable DG), demand response (DR), and interruption loads.
    \item The paper considered various operation modes to minimize total operation cost. The main contribution is to propose a detailed stochastic model.
\end{enumerate}

\textbf{DER-2017([EPSR], Olival, P.C. \& Madureira, A.G. \& Matos, M.)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{olivalAdvancedVoltageControl2017} was published in 2017. It is a centralized approach to solve a DER coordination problem for voltage control.
    \item The application scenario is DER with AC network model, considering energy storage system (ESS), RES (controllable DG), demand response (DR), and interruption loads.
    \item The paper considered various operation modes to minimize total operation cost. The main contribution is to propose a control scheme, which is a mixed strategy of power flow correction, a meta-heuristic, Evolutionary Particle Swarm method, and a sequential voltage control algorithm.
\end{enumerate}

\textbf{DER-2018-Practical([SEGN], Lipari, Gianluca \& Del Rosario, Gerard \& Corchero, Cristina \& Ponci, Ferdinanda \& Monti, Antonello)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{lipariRealtimeCommercialAggregator2018} was published in 2018. It is a practical approach for introducing aggregators for the European distribution system.
    \item The paper seems no explicit algorithm involved, and the control is coordinated and empirical. The main contribution is the interaction framework design that involves DSO, aggregator(VPP), and customers.
\end{enumerate}

\textbf{LMP-2017-Primal Parametric Programming([TPS], Ji, Yuting \& Thomas, Robert J. \& Tong, Lang)}

\begin{enumerate}[leftmargin=*]
    \item The paper \cite{jiProbabilisticForecastingRealTime2016} was published in 2017. The specific method taken is parametric programming. It is a centralized DCOPF problem.
    \item The application scenario is to find mappings of LMP w.r.t. load and generation fluctuations (parameters), considering contingency for a known time-varying topology. 
    \item The paper proposed two algorithms. One is to solve a standard MPP using the MPT toolbox. The paper explores and subdivides the parameter space into critical regions offline. 
    \item The other is dynamic critical region generation. We first use online Monte Carlo simulation to generate loads and generation as parameters randomly. If the parameter is within an explored critical region, then we find the mapping for LMP. If not, we solve a DCOPF and then find the mapping.
\end{enumerate}

==> network_mod.tex <==
%!TEX root = MainDistOptPower.tex

\subsection{Simulation data for Sections \ref{sec:multi_area}, \ref{sec:DER_coord} and \ref{sec:TD_coordination}}
\label{sec:app.data}
Network data were obtained from MATPOWER 7.1 \cite{Zimmerman2011MATPOWERSO}.

\subsubsection{Data for solving $\Pcal_1$} \label{sec:app.data.maopf}
The multi-area power system considered in Section \ref{sec:multi_area} is illustrated in Figure \ref{fig:ma.1}. 
% The topology and network parameters of internal systems are taken from \cite[Figure 7(e)]{Guo2018}.
The 118-bus networks were modified as follows. Tie-line capacities were set to $100$MW and their reactances were set to $0.25$p.u.
Capacities of transmission lines internal to each area were set to 100MW. All loads and generators at boundary buses were removed. Quadratic cost coefficients were neglected and the linear cost coefficients $\v{c}_j$ of the generators were perturbed to $\widetilde{\v{c}}_j := \v{c}_j \circ \left( 0.99 + 0.02 \v{\xi}_j \right)$, for $j = 1,\ldots,N$,
    % \begin{align}
    %     \begin{aligned}
    %     \widetilde{\v{c}}_j := \v{c}_j \circ \left( 0.99 + 0.02 \v{\xi}_j \right), \quad j = 1,\ldots,N,
    %     \end{aligned}
    % \end{align}
    where entries of $\v{\xi}_j$ are independent $\Ncal(0,1)$ (standard normal) variables. All phase angles were restricted to $[-\frac{\pi}{6}, \frac{\pi}{6}]$. 

%----------------- 2021.06.27 Update -----------------%

\subsubsection{Data for solving $\Pcal_2$} \label{sec:app.data.der}
The 4-bus network considered in Section \ref{sec:DER_coord}, shown in Figure \ref{fig:der.1}, is modified from the IEEE 4-bus network as follows. The branch joining buses 1 and 4 was altered to connect buses 3 and 4.
We enforced squared current flows as 
% $\ell_{j,k} \in [0, 2 \times 10^{-4}]\text{[}\times 10^6 \text{A}^{2}\text{]}$,
$\ell_{j,k} \in [0, 200]$ Amp$^2$,
real and reactive branch power flows as $P_{j,k} \in [-1, 1]$ MW and $Q_{j,k} \in [-1, 1]$ MVAR, respectively. 
DER generators were added at buses 2, 3 and 4. Bus 1 defined the T\&D interface. Generation capacities were fixed to $[0, 1]$ MW and $[-1, 1]$ MVAR. Generation costs were
$\alpha_{pj} (p^G_j)^2 + \beta_{pj} p^G_j + \alpha_{qj} (q^G_j)^2$ with coefficients in Table \ref{tab:cost.4}.
% \begin{align}
%     \begin{aligned}
%     c_j(p^G_j, q^G_j) = \alpha_{pj} (p^G_j)^2 + \beta_{pj} p^G_j + \alpha_{qj} (q^G_j)^2 
%     \end{aligned}
%     \label{eq:Gencost}
% \end{align}

\begin{table}[H]
\centering
% \vspace{-8pt}
\caption{Cost coefficients of the 4-bus network for $\Pcal_2$.}
\label{tab:cost.4}
\begin{tabularx}{0.45\textwidth}{c | CCCC}
    \toprule
    Bus  
    &  1  &  2  &  3  &  4  \\
    \midrule
    $\alpha_{p}$[\$/$\text{MW}^2$]  
    &  0  & 6  &  7   &  8   \\
    $\beta_{p}$[\$/MW]  
    &  30 &  19  &  18  &  17  \\  
    $\alpha_{q}$[\$/$\text{MVAR}^2$]   
    &  5  &  5.1  &  5.2  &  5.3  \\    
    \bottomrule       
\end{tabularx}
\end{table}

For the IEEE 15-bus system
shown in Figure \ref{fig:der.networks}, we modified the branch flow limits to mirror those for the 4-bus system.
We added 7 distributed generators at buses 5, 7, 8, 10, 13, 14, 15, where bus 1 is the T\&D interface, all with capacities $[0, 0.2]$ MW and $[-0.2, 0.2]$ MVAR. Generation costs were similar to the 4-bus network with coefficients in Table \ref{tab:cost.15}.
\begin{table}[H]
\centering
% \vspace{-8pt}
\caption{Cost coefficients of the 15-bus network for $\Pcal_2$.}
\label{tab:cost.15}
\begin{tabularx}{0.45\textwidth}{c | CCCCCCCC}
    \toprule
    Bus  
    &  1  &  5  & 7  & 8 & 10 & 13 & 14 & 15 \\
    \midrule
    $\alpha_{p}$[\$/$\text{MW}^2$]  
    &  0  & 25  &  23   &  21  &  19  &  17  & 15 & 13  \\
    $\beta_{p}$[\$/MW]  
    &  50 & 41  &  42   &  43  &  44  &  45  & 46 & 47  \\ 
    $\alpha_{q}$[\$/$\text{MVAR}^2$]   
    &  25 & 24  &  23   &  22  &  21  &  20  & 19 & 18  \\    
    \bottomrule       
\end{tabularx}
\end{table}

We randomized the real and reactive power demands at each change point by scaling each (real/reactive) load by 
$\left[ \omega + (\omega' - \omega) \xi \right]$,
% $\left[ a + (b - a) \xi \right]$,
% \begin{align}
%     \begin{aligned}
%     \tilde{p}^D_j = \bar{p}^D_j  \left( a_t + (b_t - a_t) \times \xi_j \right), 
%     % & \\
%     \tilde{q}^D_j = \bar{q}^D_j  \left( a_t + (b_t - a_t) \times \zeta_j \right), 
%     \end{aligned}
%     \label{eq:Load.Ptb}
% \end{align}
% $j = 1,\ldots,N$.
where $\xi\sim\Ncal(0,1)$. Parameters  $(\omega, \omega')$ were varied at the change points in the sequence $(0.70, 1.30)$, $(0.80, 1.20)$, $(0.85, 1.15)$, $(0.75, 1.20)$, $(0.95, 1.05)$. 
% per Table \ref{tab:load.change}. 
The experiment was initialized with default loads from MATPOWER.
% At each $t$, we always randomize the newest nodal active real and reactive loads. For all tests in Section \ref{sec:DER_coord}, the changes are set as
% \begin{table}[H]
% \centering
% \vspace{-8pt}
% \caption{Coefficients describing periodic load changes for $\Pcal_2$.}
% \label{tab:load.change}
% \begin{tabularx}{0.45\textwidth}{c | CCCCC}
%     \toprule
%     Change pt.
%     &  $1$  &  $2$  &  $3$  &  $4$  &  $5$ \\
%     \midrule
%     $a$
%     & 0.70 & 0.80 & 0.85 & 0.75 & 0.95 \\
%     $b$
%     & 1.30 & 1.20 & 1.15 & 1.25 & 1.05 \\       
%     \bottomrule       
% \end{tabularx}
% \end{table}

\subsubsection{Data for solving $\Pcal_3$}  \label{sec:app.data.td}
In Section \ref{sec:TD_coordination}, for the 204-bus system in Figure \ref{fig:td.1}, the 6-bus transmission network was modified as follows. All branch capacities are set to 5MW. All real and reactive generation capacities were set to $[0, 5]$MW and $[-5, 5]$ MVAR, respectively. We considered ${P}_\ell^D + j Q_\ell^D = (4 + j 4) \text{[MVA]}$ at each bus $\ell = 1,\ldots,6$. 
Generation costs were similar to the 4-bus network with coefficients in Table \ref{tab:cost.6}.
\begin{table}[H]
\centering
% \vspace{-8pt}
\caption{Cost coefficients of the 6-bus network for $\Pcal_3$.}
\label{tab:cost.6}
\begin{tabularx}{0.45\textwidth}{c | CCCCCC}
    \toprule
    Bus  
    &  1  &  2  &  3  &  4  &  5 & 6  \\
    \midrule
    $\alpha_{p}$[\$/$\text{MW}^2$]  
    &  8.7  &  5.9 &  6.8  &  7.2  &  4.2  & 3.5 \\
    $\beta_{p}$[\$/MW]  
    &  11 &  12  &  13  &  14  &  15  & 16\\  
    $\alpha_{q}$[\$/$\text{MVar}^2$]   
    & 3.2 &  3.5  &  2.3  &  1.8  &  1.5 & 1.7 \\             
    \bottomrule       
\end{tabularx}
\end{table}

For all 33-bus distribution networks, all branch capacities were set to $4$ MW. 
Four DER generators were added at buses 18, 22, 25 and 33. Bus 1 is the T\&D interface. Again, we considered generation costs as for $\Pcal_2$ but with coefficients 
$\v{\alpha}_{p\ell} = 5 \circ \left( 0.9 + 0.1  \v{\xi}_\ell \right)$, $
    \v{\beta}_{p\ell} = 20 \circ \left( 0.9 + 0.1  \v{\xi}'_\ell \right)$ and $
    \v{\alpha}_{q\ell} = 3 \circ \left( 0.9 + 0.1  \v{\xi}''_\ell \right)$
% \begin{align*}
%     \begin{aligned}
%     \v{\alpha}_{p\ell} = 5 \circ \left( 0.9 + 0.1  \v{\xi}_\ell \right), 
%     & \\
%     \v{\beta}_{p\ell} = 20 \circ \left( 0.9 + 0.1  \v{\xi}'_\ell \right), 
%     & \\
%     \v{\alpha}_{q\ell} = 3 \circ \left( 0.9 + 0.1  \v{\xi}''_\ell \right),
%     \end{aligned}
% \end{align*}
for $\ell = 1,\ldots,n^\tran$, where all entries of $\v{\xi}_\ell$, $\v{\xi}'_\ell$, $\v{\xi}''_\ell$ are drawn from $\Ncal(0,1)$. 
Real and reactive power demands in the distribution networks were randomized similarly to that for $\Pcal_2$ with $\omega=0.9$ and $\omega'=1.1$.

% At $t = 0$, the active and reactive loads for each distribution grid is perturbed according to \eqref{eq:Load.Ptb} with $a_t = 0.9$, $b_t = 1.1$, where $\bar{p}^D_j = p^D_j$, $\bar{q}^D_j = q^D_j$ are taking default values from MATPOWER.

{\color{blue}
\begin{figure}[htbp]
    \centering 
    % \vspace{.15in}
    \includegraphics[width=0.495\textwidth]{figures/td/avgdsm_eta_1e-1_iter_1e6_both.pdf}  
    % \vspace{-.2in}
    \caption{Progress of Algorithm \ref{alg:ddsa} on $\Pcal_3$ using LinDistFlow and SOCP relaxation of power flow equations for the distribution grid.
    }     
    \label{fig:td.4}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{More simulations on $\Pcal_3$}
\label{subsec:TD_socp}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Our modeling framework is flexible in that we can adopt any linearization or convex relaxation of power flow equations for the grid optimization problems. To illustrate through an example, we simulated $\Pcal_3$ with the LinDistFlow model replaced by SOCP relaxations of the power flow equations for the distribution grid, as in Section \ref{sec:DER_coord}. 
The same network in Figure \ref{fig:td.1} was considered.
We applied Algorithm \ref{alg:ddsa} with a flat start and step size $\eta = \eta_0/\sqrt{T}$, where $\eta_0 = 10^{2}$ and $T=10^{6}$.
Convergence of Algorithm \ref{alg:ddsa} with this power flow model in Figure \ref{fig:td.4} are similar to that with the LinDistFlow model. The optimal costs, however, are higher by 4.04\%, given that the SOCP relaxation model accounts for distribution losses that the LinDistFlow model does not. 
}

==> powerflow.tex <==
%!TEX root = MainDistOptPower.tex

\subsection{Primer on Various Power Flow Models}
\label{sec:powerFlow}

%================================================================

An optimal power flow (OPF) problem is an optimization problem defined over an electric power network of the following form.
\begin{align*}  
%\label{eq-OPF}
\text{minimize} \ \Ccal(\Re\{\v{s}\}), \text{subject to } \v{s} \in \Fset, {s}_i \in \Xset_i, i=1,\ldots,n.
\end{align*}
The costs $c$ depend on the application, and can encode power generation cost, disutility of deferred power consumption, etc.
$\Xset_i$ encodes the possible apparent power injections from the assets connected at bus $i$ in an $n$-bus power system. $\Fset$ denotes the set of feasible power injections, and admits different representations, depending on the power flow model. It is given by the following nonconvex set.
\begin{align} 
\label{global-constraint}
\Fset := & \{ s \in \Cset^n \ | \ s_i = \sum_{j \sim i} s_{ij}, \ s_{ij} = v^{\Hsf} \Phi^{ij} v, \ |s_{ij}| \leq f_{ij},  \notag \\
& \quad  |v_i|^2 \in [\ul{u}_i, \ol{u}_i] \text{ for some } v \in \Cset^n.  \}
\end{align}
In the above description, $j \sim i$ denotes that buses $i$ and $j$ share a line between them. The vector of voltage phasors is given by $v \in \Cset^n$, and $\Phi^{ij} \in \Cset^{n \times n}$ is a matrix with all zeros, except
$$ \Phi^{ij}_{ii} = y_{ij}^{\Hsf}, \qquad \Phi^{ij}_{ji} = - y_{ij}^{\Hsf},$$
where $y_{ij}$ denotes the admittance of the line connecting buses $i$ and $j$. Finally, $\ul{u}_i, \ol{u}_i$ define limits on (squared) voltage magnitudes at bus $i$. 

Various power flow models are adopted, depending on the application. We describe a few below.

\subsubsection{Convex relaxation of power flow models}

A second-order cone relaxation  of the AC OPF was introduced in \cite{Farivar2013,Bose2015} as a second-order cone problem (\textsf{SOCP}), which can be rewritten employing the bus injection model as follows. 
\begin{align*} 
\Fset^{\textsf{SOCP}} := & \{ s \in \Cset^n \ | \ s_i = \sum_{j \sim i} s_{ij}, \ s_{ij} = (W_{ii}-W_{ij}) \Phi^{ij},   \notag \\
& \quad  \ |s_{ij}| \leq f_{ij}, \ W_{ii} \in [\ul{u}_i, \ol{u}_i], \ W_{ii}W_{jj} \geq |W_{ij}|^2, \notag \\
& \quad \text{ for some } W \in \Cset^n. \} %, \ W \succeq 0. \}
\end{align*}


When considering the OPF problem for balanced single phase radial distribution networks, usually the branch flow model \cite{Baran1989a,Baran1989b} is utilized. In this model, we assume that each line is assigned a specific direction, i.e., the network graph becomes directed. Subsequently, we denote $z_{ij}$, $I_{ij}$, and $S_{ij}$ the complex impedance on the line $i \leftrightarrow j$, the complex current from bus $i$ to bus $j$, and the complex power sent from bus $i$ to bus $j$; respectively. Next, denote $l_{ij}\triangleq |I_{ij}|^2$ and $v_{i} \triangleq |V_{i}|^2$ which are the magnitudes of the current from 
bus $i$ to bus $j$ and of the voltage at bus $i$; respectively. Then the branch flow model representation is described by the following equations  \cite{Bose2015}.
\begin{subequations}
\begin{align}
\label{net-power}
\underline{s}_j &\leq \sum_{k:j \rightarrow k}{S_{jk}} - \sum_{i:i \rightarrow j}{(S_{ij}-z_{ij}l_{ij})} \leq \overline{s}_j, \\
\label{voltage}
0 &= v_i - v_j -2\mathrm{Re}(z_{ij}^HS_{ij}) + |z_{ij}|^2l_{ij}, \\
\label{branch-power}
|S_{ij}|^2 &\leq l_{ij}v_i,  \\
\label{volt-constrant}
\underline{v}_j &\leq v_j \leq \overline{v}_j.
\end{align}
\end{subequations}

 
This \textsf{SOCP} has also been applied to balanced radial distribution networks in \cite{Peng2018}. 


\subsubsection{DC OPF model}  When \eqref{eq-OPF} describes the economic dispatch problem in wholesale electricity markets, $\Fset$ is often approximated using a linear DC power flow model, and is given by
\begin{align*} 
\Fset^{\Dsf\Csf} := & \{ s \in \Cset^n \ | \ \Im\{s\} = 0, \ s_i = \sum_{j \sim i} s_{ij}, \\ 
& \quad \ s_{ij} = b_{ij} (\theta_i - \theta_j), \ |s_{ij}| \leq f_{ij} \text{ for some } \theta \in \Rset^n\}
\end{align*}




